For-all Sparse Recovery in Near-Optimal Time

An approximate sparse recovery system in $\ell_1$ norm consists of parameters $k$, $\epsilon$, $N$, an $m$-by-$N$ measurement $\Phi$, and a recovery algorithm, $\mathcal{R}$. Given a vector, $\mathbf{x}$, the system approximates $x$ by $\widehat{\mathbf{x}} = \mathcal{R}(\Phi\mathbf{x})$, which must satisfy $\|\widehat{\mathbf{x}}-\mathbf{x}\|_1 \leq (1+\epsilon)\|\mathbf{x}-\mathbf{x}_k\|_1$. We consider the 'for all' model, in which a single matrix $\Phi$, possibly 'constructed' non-explicitly using the probabilistic method, is used for all signals $\mathbf{x}$. The best existing sublinear algorithm by Porat and Strauss (SODA'12) uses $O(\epsilon^{-3} k\log(N/k))$ measurements and runs in time $O(k^{1-\alpha}N^\alpha)$ for any constant $\alpha > 0$. In this paper, we improve the number of measurements to $O(\epsilon^{-2} k \log(N/k))$, matching the best existing upper bound (attained by super-linear algorithms), and the runtime to $O(k^{1+\beta}\textrm{poly}(\log N,1/\epsilon))$, with a modest restriction that $\epsilon \leq (\log k/\log N)^{\gamma}$, for any constants $\beta,\gamma > 0$. When $k\leq \log^c N$ for some $c>0$, the runtime is reduced to $O(k\textrm{poly}(N,1/\epsilon))$. With no restrictions on $\epsilon$, we have an approximation recovery system with $m = O(k/\epsilon \log(N/k)((\log N/\log k)^\gamma + 1/\epsilon))$ measurements.

==> candidate.tex <==
% !TEX root = main.tex
\section{Fast Candidate Set Generation}
\label{sec:fast}

In this section, we present a structure that provides a list of
$\poly(k\log(N))$ candidate heavy hitters that includes $\Omega(k)$
true heavy hitters, in time $\poly(k\log N)$.

The general setup is as follows.  Let $B\approx (k\log N)^3$.
\mjsnote{How big does $B$ need to be, and why?}  We will hash
$h:[N]\to[B]$ at random and repeat $L=O(\log(N)/\log(B))$ times.  In
each repetition, we will recursively recover the $k$ heavy hitters in
the aggreated signal.  We will show how to recover, along with each
recovered heavy hitter, $O(\log B)$ bits of auxiliary data, defined
below, 
so that there are $\Omega(L\log B)=\Omega(\log N)$ bits of data
associated with each recovered heavy hitter.  Our main goal here is to
piece together the $L$ chunks of $\log B$ bits for position $i$ to get
$i$, which is returned as a candidate.

To store auxiliary data, one can proceed as follows.  First, to store
one additional bit $m_i$ associated with $i$, map $[B]\to[B]\times[2]$
following $h:[N]\to[B]$, deterministically, sending $i$ to
$(h(i),m_i)$.  When we recover a heavy hitter recursively from a
signal of ``length'' $[B]\times[2]$, the second component of the
position gives us $m_i$.

To store $\log(B)$ bits, we have two choices.  Either generalize the
above to map $[N]\to[B]\to[B^{O(1)}]$.  Alternatively, one can solve a
noisy set of equations modulo 2:  Each repetition gives the right hand
side for some fixed random equation in the $\log B$ bits; if enough
repetitions succeed, we will have enough equations to recover all the
bits.

\subsection{Graph Structure: Ideal, Contracted, and Implemented}

\paragraph{Expander.}

For constant $d$, pick a directed graph $G_L$ of degree $d$,
by giving each node $d$ out-arcs at random.

We now give an important property of this graph.  Note that the
following property says something about $L$ starting nodes $u$ and
$\log_d L$ possible radii from $u$, but
does {\em not} make a claim about expansion from all
exponentially-many small sets.

\begin{lemma}
\label{lem:expander}
Let $\delta=\log_d(3L)$.  Except with probability $1/\poly(L)$, for
each node $u\in G_L$, there are $.8L$ unique nodes at distance
$\delta$ from $u$ among $3L$ total endpoints of length-$\delta$
paths.
\end{lemma}
\begin{proof}
Intuitively, we proceed as follows.  Fix a starting node, $u$.  Assume
inductively that the neighborhood of $u$ at radius $j$ contains $f(j)$
unique nodes, which is about the maximum number $d^j$ of unique
nodes---in fact, assume that the neighborhood contains $f(j)\approx
d^j$ nodes that have not yet been seen at any 
radius less than $j$, either.  Then the immediate neighbors of these
are chosen independently at random from all $L$ nodes, and we can
proceed.

Our analysis treats separately the case of $f(j)<\log L$, $\log L\le
f(j)<\sqrt{L\log L}$, $\sqrt{L\log L}\le f(j)< L/d$, and $f(j)\approx
L/d$.  The reasons are indicated below by boxed expressions.

Fix distance $j$.  Let $X_r$ be the indicator variable for the $r$'th
arc ending on another node chosen during this or previous $j$.
Then $E[X_r]\le (r+d^j)/L$.  Let $X=\sum_{r\le df(j)} X_r$, so
$E[X]\approx(d^2f^2(j)/2+f(j)d^{j+1})/L\approx d^2f^2(j)/(2L)$.   As long
as $f(j)< L/d$, we
will aim for failure probability $1/L\log L$, enough to take a union
bound over all starting nodes and all distances $j$.

\begin{itemize}
\item
First, for $f(j)<0.6\log L$, consider the probability that
at least two arcs
are bad.  That means that at least two arcs collide with previous
arcs.  The probability is at most
\begin{eqnarray*}
\binom{df(j)}{2}\left(\frac{df(j)}{L}\right)^2
& \le & \frac{(df(j))^4}{L^2}\\
& \le & \frac{(0.6 d)^4 \log^{4}L}{L^2}\\
& \le & \frac1{L\log L},
\end{eqnarray*}
which is acceptably small.  The aggregate expansion over the $J$
possible $j$'s in the range $d\le f(j)<0.6\log L$ is at least
$d^J\prod_{1\le j<J}\left(1-2/d^j\right)=d^J\left(1-\frac{O(1)}d\right)\geq d^J\left(1-\frac{2.37}{d}\right)$ for $3\le d\le 10^8$.

This analysis extends for $f(j)>0.6\log L$, but only up to
\framebox{$f(j)<o\left(\frac{\sqrt{L}}d\right)$}.

\item
Now suppose $0.6\log L\le f(j)\le\frac{\sqrt{7L\log L}}d$.
 By Chernoff, we have
\[\Pr(X-E[X] > t)\le\left(\frac{e E[X]}{t}\right)^t.\]
We claim that we shall always have $f(j)\geq d^j/3$ in this case (for $d\geq 5$), and thus $f(j)\geq d^{j-1}$ and $f(j)d^{j+1}\leq d^2f^2(j)/2$, hence $E[X] \leq \frac{3}{2} d^2 f(j)^2/L$.
Since \framebox{$f(j)\le\frac{\sqrt{7L\log L}}d$} %in this case, $E[X]\approx d^2f^2(j)/(2L)\le 7\log(L)/2$
, %so that 
$eE[X]/t<0.02$ if
$t\ge 0.6\log L(\ge(21e/2)\cdot 0.02\cdot \log L)$. In that case, ($L\geq 4$ to gaurantee that $0.6\log L\geq 1$)
\[\left(\frac{e E[X]}{t}\right)^t\le (0.02)^{0.6\log L}\le 2^{-3.38\log L}<1/L\log L.\]
Here the
expansion is $f(j)$ to $df(j)-t$ to $d(df(j)-t)-t$, etc.  Rewriting,
\[df(j)-t=df(j)\left(1-\frac t{df(j)}\right)
\ge df(j)\left(1-\frac 1d\right),\]
since $t\le 0.6\log L$ and \framebox{$f(j)\ge 0.6\log L$}. The aggregate expansion for $k$ consecutive steps of this case is
\[
d^k f(j) - (d^{k-1}+\cdots +1)t = d^k f(j) \left(1-\frac{1}{d}\cdot\frac{1-d^{-J}}{1-d^{-1}}\cdot\frac{t}{f(j)}\right) \geq d^k f(j)\left(1-\frac{1}{d-1}\right) 
\]
for all $1\leq k\leq J$. Now it is easy to see the claim of a lower bound of $f(j)$ is correct, as the shrinking factor
\[
\left(1-\frac{1}{d-1}\right)\left(1-\frac{2.37}{d}\right)\geq \frac{1}{3}
\]
for $d\geq 5$.

%The expansion is
%better for larger $f(j)$ and 
%the aggregate expansion over the $J$ possible $j$'s in the range $\log
%L\le f(j)\le\sqrt{L\log L}$ is at least
%\[d^J\prod_j\left(1-\frac 1{d^j}\right)
%=d^J\left(1-\frac{O(1)}{d}\right).\]

\item
Next, suppose $\frac{\sqrt{7L\log L}}d\le f(j)\le 3L/d^2$.
Using an
alternative form of
Chernoff, we get
\[\Pr(X > (1+\epsilon)E[X])\le
e^{-\frac{\epsilon^2 E[X]}{3}}.\]
Here $E[X]\approx d^2f^2(j)/(2L)$.  Put $\epsilon=1$, so that
$1+\epsilon=2$.  Then the failure probability is
\[e^{-\frac{E[X]}{3}}\approx e^{-d^2f^2(j)/(6L)}
  \le e^{-(7/6)\log L}\le 1/L\log L,\]
using the fact that \framebox{$\frac{\sqrt{7L\log L}}d\le f(j)$}.
The expansion is from $f(j)$ to
$df(j)-(1+\epsilon)E[X]=df(j)-2E[X]$, {\em i.e.}, to
\begin{eqnarray*}
df(j)- 2E[X]
& \approx & df(j) - \frac{d^2f^2(j)}{L}\\
& = & df(j)\left(1 - \frac{df(j)}{L}\right).
\end{eqnarray*}
Here we may assume that $f(j)=3L/d^i$ for some $i$ and, because
\framebox{$f(j)\le 3L/d^2$}, we may assume $i\ge 2$.  Thus the expansion
is from $f(j)$ to $df(j)\left(1 - \frac{3}{d^i}\right)$
for some $i\ge 1$ and $i(j+1)=i(j) + 1$.  Thus the aggregrate
expansion over all
$J\approx
\log_d(3L/d^2) - \log_d\left(\frac{\sqrt{7L\log L}}d\right) + 1$ of the
$j$'s in the range $\frac{\sqrt{7L\log L}}d\le f(j)\le 3L/d^2$ is at
least
\[d^J\prod_{i\ge 1}\left(1 - \frac{3}{d^i}\right)\ge
d^J\left(1 - \frac{O(1)}d\right).\]

\item
Finally, suppose $f(j)\approx 3L/d$, by making $L$ approximately $1/3$
times a power of $d$.  (Note that $f(j-1)\approx 3L/d^2$ is
handled by the previous case.)  The idea is that even if a path collides with
another path from this or a previous distance, we will count
the affected node once, giving up on the independence of extensions
that we needed earlier but do not need for the last step.  We will
tolerate many more collisions---most of the $3L$ paths will collide,
since there are only a total of $L$ possible unique endpoints---in
order to get a large fraction of nodes hit.  This means that expansion
will be $.8L / (3L/d) \approx d/4$, which is much worse than the $d(1-1/d)$
that we achieved at previous steps, so we can only afford this
analysis for \framebox{at most $O(1)$ possible $j$'s}.
Proceeding, each of the $L$ nodes is uncovered with
probability $(1-1/L)^{3L}\approx e^{-3}\approx 1/20$.
Nodes are left uncovered with negative correlation, so we can use the
arithmetic and Chernoff bound as for independent events.  We expect
$\mu\le L/20$ uncovered nodes and get $L/5=L-.8L$ uncovered nodes,
{\em i.e.} we get $t=(3/20)L$ more than the expected number, with
probability at most
\[\left(\frac{e\mu}{t}\right)^{t}\approx .9^t\approx .985^L<1/L\]
and $1/L$ is small
enough to take a union bound over starting nodes.  (No need for
$1/L\log L$ here.)  The aggregate expansion factor over the
previous stages is $(1-O(1)/d)$ times the design maximum, and we can
ignore that factor, getting $.8L$ unique nodes out of a total of
around $3L$ paths.
\end{itemize}

(Note: $.985^L<1/L$ if $\log(N)/\log B = L\ge 400$, {\em i.e.}, if
$N\ge B^{400}=(k\log N)^{1200}$, which, for $k=2$, occurs for $N\ge
2^{20,000}\approx10^{6000}$ or so.  No attempt has been made here to
optimize these constants.)
\end{proof}

\paragraph{Definitions of Our Graphs.}

Let $G_{LN}$ be a directed graph on $LN$ nodes, regarded as $L$ rows and
$N$ columns.  Each column of $G_{LN}$ is a copy of $G_L$.  Thus all
arcs of $G_{LN}$ are within the same column.

Now we defined a contracted version of node names.  For $B'=\poly(B)$,
partition the $r$'th row of $G_{LN}$ randomly into $B'$ pieces, by
giving each node $(r,i)$ a $\log(B')$-bit random string $p(r,i)$.  
The {\em contracted name} of node $(r,i)\in
G_{LN}$ is $(r,p(r,i))$.

Now define a graph, $G_{LB'}$.  It has $L$ rows and $B'$ nodes in each
row, defined as the partition pieces.  Formally, the nodes are of the
form $(r,p)$, where $p$ is some value taken by the function $p(r,i)$
for some $i$.  For each arc $(r,i)\to(r',i)\in G_{LN}$, put an arc
$(r,p(r,i))\to(r',p(r',i))\in G_{LB'}$.

Note that, in $G_{LB'}$, we can no longer regard the set of nodes as
an $L$-by-$B'$ rectangle, only as a collection of $L$ rows, each with
$B'$ nodes.  There is no notion of column in $G_{LB'}$, and so its
arcs are not confined to columns.  There may be parallel arcs.  The
number of nodes is $LB'$, a small number, but the
total number of arcs (counting parallel arcs multiply) is $dLN$, a
large nubmer, the
same in $G_{LB'}$ as in $G_{LN}$.

\paragraph{Implementation as Measurement Matrix.}

We now show how to use the $O(\log B)$ auxiliary bits to encode
$G_{LB'}$.  Specifically, for a node $(r,i)$ pointing to $(r',i)$,
where $r$ and $r'$ are rows and $i$ is a column, we store the
contracted names $p(r,i)$ and $p(r',i)$ among the $O(d\log B)$
auxiliary bits of $i$ in repetition $r$.  It will turn out that the
rows $r$ and $r'$
can be recovered at runtime, and do not need to be stored.  Thus,
intuitively, $r$ is known, then $p(r,i)$ gives partial information
about $i$, so that $(r,p(r,i))$ is partial information about $(r,i)$.
This is a lossless encoding of $G_{LB'}$, with $LB'$ nodes and $dLN$
arcs.

\paragraph{Runtime Graph.}

Finally, we define a noisy runtime version $\widetilde G_{LB'}$ of
$G_{LB'}$.  The nodes of $\widetilde G_{LB'}$ have names of the form $(r,p)$,
just like $G_{LB'}$.  When we do recursive recovery, in repetition
$r$, we recover some node by its contracted name, $p$, encoded in
the auxiliary bits.  Since we know what repetition $r$ the algorithm
is in, we have learned $(r,p)$.  We 
also recover arcs out of that node, in contracted form.  That is,
using $r$ and $G_L$ to learn some $r'$, we get $(r',p')$, where
$p'=p(r',i')$ for some $i'$, and $p'$ is also stored in the auxiliary
bits.  Put
the arc $(r,p)\to(r',p')$ into
$\widetilde G_{LB'}$.  Thus, if recursive recovery returns $k'$
putative heavy hitters in each of $L$ repetitions, there are $dLk'$
arcs in $\widetilde G_{LB'}$, and the entire graph $\widetilde
G_{LB'}$ is small enough that we can consume time polynomial in its
size.

Note that if recursive recovery produces $i\ne i'$ with
$p(r,i)=p(r,i')$, then one of these recoveries is incorrect.  Discard
$(r,p(r,i))=(r,p(r,i'))$ as a node detected to have failed.

\subsection{Recovery Algorithm}

\paragraph{Intuition.}

If all goes well, a node $(r,p)\in\widetilde G_{LB'}$ is dominated by
a single heavy hitter $i$, such that $(r,p)=(r,p(r,i))$.  We then use
arcs out of $(r,i)\in G_{LN}$ as the basis for arcs out of
$(r,p(r,i))\in \widetilde G_{LB'}$.  Our goal here is to show that,
for enough heavy hitters $i$, there are $\Omega(L)$ good nodes
$(r,p(r,i))\in \widetilde G_{LB'}$, {\em i.e.}, dominated by $i$,
that we can link together with each other and with at most a small
fraction of $L$ bad nodes.  Then we can use error-correcting codes to
get $i$ from the collection of $\log N$ bits with a small constant
fraction of errors.

\paragraph{Challenge.}

We need failure probability around $1/N^k$ overall, or about
$1/N\approx 1/B^L$ for each $i$.  Each node fails with probability
around $1/\poly(B)$, so we need to consider $\Omega(L)$ nodes at a
time to form an event with small enough probability.  We cannot
directly link nodes in $\widetilde G_{LB'}$ by walking from one node
to an immediate neighbor.  Also, it is likely enough that $\widetilde
G_{LB'}$ contains a large component of $\Omega(kL)$ nodes and some
isolated nodes, so we cannot link nodes in $\widetilde G_{LB'}$ by
taking directed components---this would be not much better than taking
all nodes in $\widetilde G_{LB'}$.  We need an appropriate notion of
strong connectivity, that we define next.

\paragraph{Algorithm, formally.}

For each node $(r,p)\in\widetilde G_{LB'}$, do a breadth first search
of depth $\delta=\log_d (3L)$, getting exactly $3L$ paths of length
$\delta$.  Call the multiset of nodes at path endpoints the
{\em ($\delta$-out-) neighborhood} of $(r,p)$.  If the neighborhood has
more than $1.01L$ unique nodes, discard $(r,p)$.  Otherwise, put a
node $v$ into the cluster $C_u$ of a starting node $u$ if the
neighborhoods of $u$ and $v$ intersect in at least $.58L$ nodes.

Below, we will show that clusters for many different $i$ have at least
$cL$ nodes
dominated by the same $i$ and at most $c'L$ other nodes, where $c'<c$
are constants so that error-correcting codes can correct the
$c'L\log(B)$ bits in error and produce the $O(L\log B)=\log N$ bits in
the name of $i$.

\paragraph{Algorithm, formally---Error-Correcting Code.}

We will use error-correcting codes that
tolerate many erasures (much more than half), since we are recovering
$cL$ nodes,
which is a small fraction of all $L$ nodes for that heavy hitter.
Reed-Solomon may work here:  We recover $cL$ points on a low-degree
polynomial, of which $c'L$ are in error, for constant $c'$ much
smaller than $c$.  We do not know in advance which points on the
polynomial will be recovered, but Berlekamp-Welch Reed-Solomon
decoding works in this model.
(See http://people.csail.mit.edu/madhu/FT02/slides/lect11slx4.pdf.)

That is, we want to encode $\log(N)$ bits, as $m=\log(N)/\log(B)$
chunks of $O(\log B)$ bits each, regarded as an element of a field of
size $q=\poly(B)$.  Use a polynomial $f$ of degree
$m-1$ over the field of size $q$ to enocde the $m$
chunks.  Let $t=c'L$ be a bound on the number of errors.  Evaluate $f$ at
$L\ge m+2t$ points; note that $q>L$.  If we recover $m+2t=cL$ points of
which at most $t$ are wrong, then the recovered points $y$ satisfy
$g=y\psi$, where $g$ is a polynomial of degree $m+t-1$ and $\psi$
is the error locator polynomial, non-zero of degree at most $t$,
that is zero at the errors.  The $m+2t$ evaluations are enough to find
the $m+2t$ total coefficients in $g$ and $\psi$.  This is a linear system, that
has a solution (as we just argued).  The solution $(g,\psi)$ is not
necessarily
unique---for example, if the actual number $e$ of errors is much less
than $t$ (including even $e=0$) then $\psi$ is a degree-$t$
polynomial constrained only to 
be zero on some set of $e<t$ points.  Starting with a solution in
which the degree of $y$ is only $e$ and the degree of $g$ is at most
$m+e-1$, we can multiply $g$ and $\psi$ by the same polynomial of degree
$t-e$ and get a new solution.  Even if $e=t$, we can multiply $g$ and
$\psi$ by the same constant to get a new solution, and $(g,y)=(0,0)$ is a
solution.  But we insist on a non-zero solution from the
$(t-e+1)$-dimensional space of solutions and any non-zero solution works.
%% But $g/\psi$ is invariant over
%% the solutions $(g,\psi)$:  If $g=y\psi$ 
%% and $g'=y\psi'$, then $gy\psi'=g'y\psi (= gg')$.  If
%% $y$ is 
%% not 0 at some $i$, then, canceling $y$, we see that $g\psi'=g'\psi$
%% there.  On the other hand, if $y$ is $0$ at some
%% $i$, then the error-locator polynomials $\psi$ and $\psi'$ are 0
%% there, too, so that $g\psi'=g'\psi(=0)$ there.  Since $g\psi'$ agrees
%% with $g'\psi$ on $m+2t$ points and they have degree $m+2t-1$, they are
%% equal.
Since $\psi\not\equiv 0$ and $\psi$ has degree $t$, there
remain $m+t$ points where $\psi$ is not zero, which are non-errors, so
we can interpolate $f$ from $y$ at these points.


\subsection{Correctness Proof}

\paragraph{Basic Arithmetic and Intuition.}

Above we showed tight control over the out-degree of the expander
$G_L$.  Suppose for now that the expander also has very close to $d^j$
nodes {\em preceeding} each given node by $j$ steps.  Then the total
number of paths is $3L^2$, since each of $L$ starting nodes has
$3L$ paths.  For each $j\le\delta=\log_d N$, a bad node $\nu$ has at
most $d^{\delta-j}$ path extensions of length $\delta-j$ and (by our
heroic assumption) $\nu$ is the $j$'th node of exactly $d^j$ starting
nodes.  Taking a union over all $j$, each bad node can then ruin
$d^{\delta-j}\cdot d^j\cdot\delta= O(L\log_d L)$ paths.  Each of $L$
nodes fails more or less independently with probability $1/B\le
c/\log_d L$, so we can arrange that there are at most $L/\log B$ bad
nodes except with acceptable probability.  So the number of ruined
paths is $L\log_d L\cdot L/\log B$, which we can arrange to be a small
constant fraction of the total number $3L^2$ of paths.

\paragraph{Bounding in-degrees.}

Unfortunately, the in-degrees are not so tightly bounded.  Let $X_u$
be the in-degree of $u$ if $u$ fails and $X_u=0$, otherwise, and let
$X=\sum_u X_u$.  Then,
since nodes fail effectively independently and the average
distance-$j$ in-degree equals the average (and concentrated)
distance-$j$ out-degree, which is at most $d^j$ even in the recovered
graph $\widetilde G_{LB'}$, we conclude that $E[X]$ is the same in
the constant-in-degree graph as in the real $\widetilde G_{LB'}$.
Furthermore, each in-degree (at any distance
$j$) is at most $L$ in $\widetilde G_{LB'}$ and at least $1$ in the
constant-in-degree graph, so the variance of $X$ in $\widetilde
G_{LB'}$ is at most $L^2$ times the variance of $X$ in the ideal
graph.  We can accomodate the increased
variance by increasing $B$ by the factor $L^2<\log^2 N$, which leaves
$B$ of the form $(k\log N)^{O(1)}$. 

Thus, fixing $j$ and letting $X$ be the sum over all $O(kL)$ recovered
nodes of $X_u$'s as above, we have $E[X]=d^jkL/B$ and
\[\Pr(X - E[X] > t)\le \left(\frac{eE[X]}{t}\right)^t,\]
which is at most $1/N$ if $t\approx d^jkL/\log B$.  Thus we may assume
that, for {\em each} $j$, there are at most $d^jkL/\log B$ total
paths of length $j$ {\em to} bad nodes.  Each bad node also has
distance-$(\delta-j)$ out-degree close to $d^{\delta-j}$, so, for each
$j$, the total number of paths incident on bad nodes at position $j$
may be assumed to be at most $kL^2/\log(B)$.  Taking a union over all
$\log L$ values of $j$, the total number of paths incident on bad
nodes is at most some small constant fraction of the total number of
paths, $kL^2$.

\paragraph{Final Arithmetic.}

In the good case, a node has at least $.8L$ paths to unique nodes
with the same $i$, at most $0.01L$ paths to nodes with different $i$, and
the remainder of the paths are to duplicates of nodes with the same $i$.
Call such nodes {\em $i$-well-connected}.  Note that a node can only be
$i$-well-connected with a single $i$.  An $i$-well-connected and an
$i'$-well-connected node have
intersection size at least $(2\cdot(.8-.01)-1)L=.58L$ or at most
$0.01L$, depending on whether or not $i=i'$.

Thus a cluster $C_u$ consists of {\em good} nodes that are dominated
by some $(r,p(r,i))$ and also $i$-well-connected, and an arbitrary
number of {\em bad} nodes $\nu$ that are {\em not} of that form but
nevertheless $\nu$ has neighborhood intersection with $u$ of size at
least $.58L$ because at least $.58L$ of $\nu$'s paths are bad.  But, for
each such $\nu$, there can be at most one such $i$, because at least
half of $\nu$'s neighborhood is pledged to that $i$.  A cluster for
some $i$ is recoverable even if
it has as many as, say, $L/10$ bad nodes in it.  Each bad node in that
cluster accounts for at least $.58L>L/2$ paths, for a total of at least
$L^2/20$ paths associated with an unrecoverable $i$.  Since the total
number of paths is at most, say, $kL^2/100$, at most $k/5$ of the
$i$'s can be unrecoverable, leaving $\Omega(k)$ recoverable.


==> macro-file.tex <==
%&LaTeX

%%% This document contains macros that will be used throughout
%%% It is very neatly organized.


%%%%% Packages
\usepackage{amsmath,amsthm,amsfonts,amscd}
\usepackage{amssymb}
\usepackage{bm}
%\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage[mathcal]{eucal}
%\usepackage{verbatim}
%\usepackage{url}
%\usepackage{color}
%\usepackage{supertabular}
\usepackage{multirow}
%\usepackage{algorithmic}
\usepackage{algorithmicx,algpseudocode}

\algloopdefx{NFor}[1]{\textbf{for} #1 \textbf{do}}
\algloopdefx{NIf}[1]{\textbf{if} #1 \textbf{then}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\newtheoremstyle{newthm}
  {3pt} % Space above
  {3pt} % Space below
  {\itshape} % Body font
  {} % Indent amount
  {\bfseries} % Theorem head font
  {.} % Punctuation after theorem head
  {.5em} % Space after theorem head
  {} % Theorem head spec (can be left empty, meaning `normal')
\theoremstyle{newthm}   

\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{problem}[theorem]{Problem}
\newtheorem*{problem*}{Problem}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}

\newreptheorem{theorem}{Theorem}

\newtheoremstyle{newdef}
  {2pt} % Space above
  {2pt} % Space below
  {} % Body font
  {} % Indent amount
  {\bfseries} % Theorem head font
  {.} % Punctuation after theorem head
  {.5em} % Space after theorem head
  {} % Theorem head spec (can be left empty, meaning `normal')
\theoremstyle{newdef} 

%\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
%%% Theorem setup

%\theoremstyle{plain}

\newtheorem{bigthm}{Theorem}
\renewcommand{\thebigthm}{\Alph{bigthm}}	% Number with A, B, C, etc.
%\newtheorem{thm}{Theorem}
%\newtheorem{claim}{Claim}
%\newtheorem{cor}[thm]{Corollary}
%\newtheorem{lemma}[thm]{Lemma}
%\newtheorem{prop}[thm]{Proposition}
%\newtheorem{fact}[thm]{Fact}
%\newtheorem{definition}[thm]{Definition}
%\newtheorem{invariant}[thm]{Invariant}

%\theoremstyle{definition}
%\newtheorem{algorithm}[thm]{Algorithm}
%\newtheorem{rem}[thm]{Remark}
\numberwithin{equation}{section}
%%%  Martin's macros

%%%  Counters for theorems and lemmas whose proofs are in appendix:

\newenvironment{reflemma}[1]{\medskip\parindent 0pt{\bf Lemma \ref{#1}}\em }{\vspace{1em}}
\newenvironment{reftheorem}[1]{\medskip\parindent 0pt{\bf Theorem \ref{#1}}\em }{\vspace{1em}}



%%% Typesetting

\DeclareMathAlphabet{\mathsfsl}{OT1}{cmss}{m}{sl}


%%% Other font changes

\newcommand{\lang}{\textit}
\newcommand{\titl}{\textsl}
\newcommand{\term}{\emph}
\newcommand{\algname}{\textsc}
\newcommand{\notate}[1]{\textcolor{red}{\textbf{[#1]}}}
\newcommand{\movenote}[1]{\textcolor{blue}{\textbf{[#1]}}}
\newcommand{\cnst}[1]{\mathrm{#1}}


%%% New environments

%\newenvironment{inputs}%
%	{\makebox{\phantom{}} \\ %
%		\textsc{Input:}\begin{itemize}}%
%	{\end{itemize}}
%
%\newenvironment{outputs}%
%	{\textsc{Output:}\begin{itemize}}%
%	{\end{itemize}}
%
%\newenvironment{procedure}%
%	{\textsc{Procedure:}\begin{enumerate}}%
%	{\end{enumerate}}

%%% Old symbols with new names

%\newcommand{\oldphi}{\phi}
%\renewcommand{\phi}{\varphi}
%\newcommand{\eps}{\varepsilon}


%%% New symbols

%\newcommand{\defby}{\overset{\mathrm{\scriptscriptstyle{def}}}{=}}
%\newcommand{\half}{\tfrac{1}{2}}
%\newcommand{\third}{\tfrac{1}{3}}



%%% Constants

%\newcommand{\econst}{\mathrm{e}}
%\newcommand{\iunit}{\mathrm{i}}
%\newcommand{\onevct}{\mathbf{e}}
%\newcommand{\zerovct}{\vct{0}}
%\newcommand{\Id}{\mathbf{I}}
%\newcommand{\onemtx}{\bm{1}}
%\newcommand{\zeromtx}{\bm{0}}


%%% Sets

%\newcommand{\coll}[1]{\mathscr{#1}}
%
%\newcommand{\Sspace}[1]{\mathbb{S}^{#1}}
%
%\newcommand{\Rplus}{\mathbb{R}_{+}}
%\newcommand{\Rspace}[1]{\mathbb{R}^{#1}}
%\newcommand{\Cspace}[1]{\mathbb{C}^{#1}}
%
%\newcommand{\RPspace}[1]{\mathbb{P}^{#1}(\mathbb{R})}
%\newcommand{\CPspace}[1]{\mathbb{P}^{#1}(\mathbb{C})}
%\newcommand{\FPspace}[1]{\mathbb{P}^{#1}(\mathbb{F})}
%
%\newcommand{\RGspace}[2]{\mathbb{G}( {#1}, \Rspace{#2} )}
%\newcommand{\CGspace}[2]{\mathbb{G}( {#1}, \Cspace{#2} )}
%\newcommand{\FGspace}[2]{\mathbb{G}( {#1}, \mathbb{F}^{#2} )}
%
%\newcommand{\RR}{$\Rspace{}$}
%\newcommand{\CC}{$\Cspace{}$}
%
%\newcommand{\Mset}[1]{\mathbb{M}_{#1}}
%
%\newcommand{\polar}{\circ}

%%% Real and complex analysis

\newcommand{\abs}[1]{\left\vert {#1} \right\vert}
\newcommand{\abssq}[1]{{\abs{#1}}^2}

\newcommand{\sgn}[1]{\operatorname{sgn}{#1}}
\newcommand{\real}{\operatorname{Re}}
\newcommand{\imag}{\operatorname{Im}}

\newcommand{\diff}[1]{\mathrm{d}{#1}}
\newcommand{\idiff}[1]{\, \diff{#1}}

\newcommand{\grad}{\nabla}
\newcommand{\subdiff}{\partial}

\newcommand{\argmin}{\operatorname*{arg\; min}}
\newcommand{\argmax}{\operatorname*{arg\; max}}


%%% Probability

\newcommand{\Prob}[1]{\operatorname{\mathbb{P}}\left\{ {#1} \right\}}
\newcommand{\Expect}{\operatorname{\mathbb{E}}}

\newcommand{\normal}{\textsc{normal}}
\newcommand{\erf}{\operatorname{erf}}



%%% Vector and matrix operators

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}
%\newcommand{\mtx}[1]{\mathsfsl{#1}}


\newcommand{\transp}{T}
\newcommand{\adj}{*}
\newcommand{\psinv}{\dagger}

\newcommand{\lspan}[1]{\operatorname{span}\{{#1}\}}

\newcommand{\range}{\operatorname{range}}
\newcommand{\colspan}{\operatorname{colspan}}

\newcommand{\rank}{\operatorname{rank}}

\newcommand{\diag}{\operatorname{diag}}
\newcommand{\trace}{\operatorname{trace}}

\newcommand{\supp}[1]{\operatorname{supp}(#1)}

\newcommand{\smax}{\sigma_{\max}}
\newcommand{\smin}{\sigma_{\min}}

\newcommand{\restrict}[1]{\big\vert_{#1}}

%%% Mensuration: inner products and norms

\newcommand{\ip}[2]{\left\langle {#1},\ {#2} \right\rangle}
\newcommand{\absip}[2]{\abs{\ip{#1}{#2}}}
\newcommand{\abssqip}[2]{\abssq{\ip{#1}{#2}}}
\newcommand{\tworealip}[2]{2 \, \real{\ip{#1}{#2}}}

\newcommand{\norm}[1]{\left\Vert {#1} \right\Vert}
\newcommand{\normsq}[1]{\norm{#1}^2}

	% Fixed-size inner products and norms are useful sometimes

\newcommand{\smip}[2]{\bigl\langle {#1}, \ {#2} \bigr\rangle}
\newcommand{\smabsip}[2]{\bigl\vert \smip{#1}{#2} \bigr\vert}
\newcommand{\smnorm}[2]{{\bigl\Vert {#2} \bigr\Vert}_{#1}}

\newcommand{\enorm}[1]{\norm{#1}_2}
\newcommand{\enormsq}[1]{\enorm{#1}^2}

\newcommand{\fnorm}[1]{\norm{#1}_{\mathrm{F}}}
\newcommand{\fnormsq}[1]{\fnorm{#1}^2}

\newcommand{\pnorm}[2]{\norm{#2}_{#1}}
\newcommand{\infnorm}[1]{\norm{#1}_{\infty}}

\newcommand{\iinorm}[1]{\pnorm{\infty,\infty}{#1}}

\newcommand{\rxnorm}[1]{\pnorm{\mathrm{rx}}{#1}}

\newcommand{\triplenorm}[1]{\left\vert\!\left\vert\!\left\vert {#1} \right\vert\!\right\vert\!\right\vert}

\newcommand{\dist}{\operatorname{dist}}

\newcommand{\serr}[1]{\left\| #1 \right\|_{\sim}}
\newcommand{\nerr}[1]{\left\| #1 \right\|}

%%% Unusual operators

\newcommand{\cover}{\operatorname{cover}}
\newcommand{\pack}{\operatorname{pack}}
\newcommand{\maxcor}{\operatorname{maxcor}}
\newcommand{\ERC}{\operatorname{ERC}}
\newcommand{\quant}{\operatorname{quant}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\spark}{\operatorname{spark}}

\DeclareMathOperator{\Var}{Var}

\newcommand{\identify}{{\rm identify}}
\newcommand{\estimate}{{\rm estimate}}
\newcommand{\dosketch}{{\rm sketch}}

\newcommand\rtp{{\otimes_{{\rm r}}}}
\newcommand\rds{{\oplus_{{\rm r}}}}
\newcommand\sdp{{\ltimes_{{\rm r}}}}
\newcommand\hp{{\odot}}

%%% Problem Names

\newcommand{\exactprob}{\textsc{(exact)}}
\newcommand{\rexact}{\textsc{(r-exact)}}
\newcommand{\errorprob}{\textsc{(error)}}
\newcommand{\rerror}{\textsc{(r-error)}}
\newcommand{\sparseprob}{\textsc{(sparse)}}
\newcommand{\subsetprob}{\textsc{(subset)}}
\newcommand{\rsubset}{\textsc{(r-subset)}}

\newcommand{\lonepen}{\textsc{($\ell_1$-penalty)}}
\newcommand{\loneerr}{\textsc{($\ell_1$-error)}}


%%% Things that get typed a lot

\newcommand{\Dict}{\coll{D}}

\newcommand{\opt}{\mathrm{opt}}
\newcommand{\bad}{\mathrm{bad}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\alt}{\mathrm{alt}}
\newcommand{\good}{\mathrm{good}}

\newcommand{\subjto}{\quad\text{subject to}\quad}
\newcommand{\etal}{et al.\ }

\newcommand{\cost}[2]{\operatorname{cost}_{#1}(#2)}

\newcommand{\TF}{\mathrm{TF}}

\newcommand{\chord}{\mathrm{chord}}
\newcommand{\proj}{\mathrm{spec}}
\newcommand{\fs}{\mathrm{FS}}

\newcommand{\signal}{{\mathbf x}}
\newcommand{\signalb}{{\mathbf B}}
\newcommand{\signalc}{{\mathbf C}}
\newcommand{\signale}{{\mathbf E}}
\newcommand{\signalf}{{\mathbf F}}
\newcommand{\signalg}{{\mathbf G}}
\newcommand{\signalh}{{\mathbf H}}
\newcommand{\filter}{{\zeta}}
\newcommand{\signals}{{\mathbf S}}
%\newcommand{\repn}{{\mathbf R}}
\newcommand{\repn}{{\mathbf r}}
\newcommand{\signala}{{\mathbf a}}
\newcommand{\noise}{{\nu}}

%%% Constants, vectors and matrices with names

%\newcommand{\atom}{\vct{\phi}}
%\newcommand{\Fee}{\mtx{\Phi}}
%
%\newcommand{\Lamopt}{\Lambda_{\opt}}
%
%\newcommand{\astar}{\vct{a}_{\star}}
%\newcommand{\aLam}{\vct{a}_{\Lambda}}
%\newcommand{\aopt}{\vct{a}_{\opt}}
%
%\newcommand{\Astar}{\mtx{A}_{\star}}
%\newcommand{\ALam}{\mtx{A}_{\Lambda}}
%\newcommand{\Aopt}{\mtx{A}_{\opt}}
%
%\newcommand{\cLam}{\vct{c}_{\Lambda}}
%\newcommand{\copt}{\vct{c}_{\opt}}
%
%\newcommand{\CLam}{\mtx{C}_{\Lambda}}
%\newcommand{\Copt}{\mtx{C}_{\opt}}
%
%\newcommand{\bstar}{\vct{b}_{\star}}
%\newcommand{\bLam}{\vct{b}_{\Lambda}}
%\newcommand{\bbad}{\vct{b}_{\bad}}
%\newcommand{\balt}{\vct{b}_{\alt}}
%\newcommand{\bopt}{\vct{c}_{\opt}}
%
%\newcommand{\Bstar}{\mtx{B}_{\star}}
%\newcommand{\BLam}{\mtx{B}_{\Lambda}}
%\newcommand{\Bopt}{\mtx{B}_{\opt}}
%\newcommand{\Balt}{\mtx{B}_{\alt}}
%
%\newcommand{\Ropt}{\mtx{R}_{\opt}}
%
%
%\newcommand{\gamstar}{\gamma_{\star}}
%
%\newcommand{\PhiLam}{\mtx{\Phi}_{\Lambda}}
%\newcommand{\Phiopt}{\mtx{\Phi}_{\opt}}
%\newcommand{\Phialt}{\mtx{\Phi}_{\alt}}
%\newcommand{\Psiopt}{\mtx{\Psi}}
%\newcommand{\PsiLam}{\mtx{\Psi}_{\Lambda}}
%
%
%\newcommand{\Popt}{{\mtx{P}_{\opt}}}
%\newcommand{\PLam}{{\mtx{P}_{\Lambda}}}
%
%\newcommand{\GLam}{{\mtx{G}_{\Lambda}}}
%
%\newcommand{\rhoerr}{\rho_{\err}}
%\newcommand{\rhoopt}{\rho_{\opt}}
%
%\newcommand{\success}{\mathrm{succ}}
%\newcommand{\failure}{\mathrm{fail}}

\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}

%%%%% Stupid LaTeX tricks

%\newcommand{\forcetall}{\phantom{\frac{1}{\frac{1}{1}}}}


%%%%%%%%%%%%%%%%%%%%%%%


%% Added by mjs:

\DeclareMathOperator{\med}{med}

